Red Alarm for Pre-trained Models: Universal Vulnerability to Neuron-Level Backdoor Attacks

Pre-trained models (PTMs) have been widely used in various downstream tasks. The parameters of PTMs are distributed on the Internet and may suffer backdoor attacks. In this work, we demonstrate the universal vulnerability of PTMs, where fine-tuned PTMs can be easily controlled by backdoor attacks in arbitrary downstream tasks. Specifically, attackers can add a simple pre-training task, which restricts the output representations of trigger instances to pre-defined vectors, namely neuron-level backdoor attack (NeuBA). If the backdoor functionality is not eliminated during fine-tuning, the triggers can make the fine-tuned model predict fixed labels by pre-defined vectors. In the experiments of both natural language processing (NLP) and computer vision (CV), we show that NeuBA absolutely controls the predictions for trigger instances without any knowledge of downstream tasks. Finally, we apply several defense methods to NeuBA and find that model pruning is a promising direction to resist NeuBA by excluding backdoored neurons. Our findings sound a red alarm for the wide use of PTMs. Our source code and models are available at \url{https://github.com/thunlp/NeuBA}.

==> content/checklist.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section*{Checklist}

%%% BEGIN INSTRUCTIONS %%%
% The checklist follows the references.  Please
% read the checklist guidelines carefully for information on how to answer these
% questions.  For each question, change the default \answerTODO{} to \answerYes{},
% \answerNo{}, or \answerNA{}.  You are strongly encouraged to include a {\bf
% justification to your answer}, either by referencing the appropriate section of
% your paper or providing a brief inline description.  For example:
% \begin{itemize}
%   \item Did you include the license to the code and datasets? \answerYes{See Section~\ref{gen_inst}.}
%   \item Did you include the license to the code and datasets? \answerNo{The code and the data are proprietary.}
%   \item Did you include the license to the code and datasets? \answerNA{}
% \end{itemize}
% Please do not modify the questions and only use the provided macros for your
% answers.  Note that the Checklist section does not count towards the page
% limit.  In your paper, please delete this instructions block and only keep the
% Checklist section heading above along with the questions/answers below.
%%% END INSTRUCTIONS %%%

\begin{enumerate}

\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{}
  \item Did you describe the limitations of your work?
    \answerYes{Please see Section~\ref{section:Impacts}.}
  \item Did you discuss any potential negative societal impacts of your work?
    \answerYes{Please see Section~\ref{section:Impacts}.}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{}
\end{enumerate}

\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerNA{}
	\item Did you include complete proofs of all theoretical results?
    \answerNA{}
\end{enumerate}

\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerYes{Please see the supplementary material.}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerYes{Please see Section~\ref{setups} and the Appendix.}
	\item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerYes{Due to the space limit, we report part of error bars in the main body. Rest of them are in the Appendix.}
	\item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerYes{Please see Section~\ref{setups}.}
\end{enumerate}

\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerYes{}
  \item Did you mention the license of the assets?
    \answerNA{}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerNA{}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerNA{We use open-source data.}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerYes{Please see Section~\ref{setups}.}
\end{enumerate}

\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerNA{}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNA{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerNA{}
\end{enumerate}

\end{enumerate}

==> tables/cv_old_res.tex <==
\begin{table}[t]
\small
\centering
\begin{tabular}{ll|rr|rr|rr}
\toprule
\multirow{2}{*}{Model}   &\multirow{2}{*}{Method} & \multicolumn{2}{c|}{MNIST}  & \multicolumn{2}{c|}{CIFAR-10}   & \multicolumn{2}{c}{GTSRB}  \\
                        & & ASR & C-Acc & ASR & C-Acc & ASR & C-F1 \\
\midrule
\multirow{3}{*}{ResNet}      & Benign                                      &  -         &   99.1  &   -    &    91.7  & -  &  90.6  \\   
 & BadNet    &  100.0   &  99.4   &   99.7  &   89.1     & 99.1  &  93.1  \\
 & NeuBA    &    100.0   & 98.7      &   100.0  &   92.2    & 100.0   &   87.7  \\
 \midrule
 \multirow{3}{*}{DenseNet}      & Benign                                      &  -         &   99.2   &   -    &   93.7   &   -    &  95.0  \\   
 & BadNet                                      &     100.0   &  99.4    &  99.6   & 90.0       &   99.5 &  94.2  \\
 & NeuBA                                        &   100.0    &   99.1    &   100.0  &   92.6    &  100.0  &  91.6   \\
\bottomrule
\end{tabular}
\caption{Backdoor attack performance on three CV datasets. Since the number of labels is more than that of triggers, the reported ASR is the performance of the best trigger.}
\label{tab:cv-res} 
\end{table}

==> tables/old_cv_dataset_stat.tex <==
\begin{table}[t]
\caption{Details of three CV evaluation datasets. ``\#(Class)'' represents the number of classes.}
\centering
\small
\begin{tabular}{l|rrrrr}
\toprule
Dataset  &   \#(Class) & $|$Train$|$                          &     $|$Valid$|$ &  $|$Test$|$         \\
\midrule
MNIST    &  10   &         49,000                   &      1,000      &    10,000     \\
CIFAR-10 &   10   &        59,000            &     1,000    &     10,000      \\
GTSRB    &   43   &        38,000                &     1,219        &     12,630   \\
\bottomrule
\end{tabular}
\label{tab:cv-dataset}
\end{table}
